Few-Shot Domain Adaptation for Named-Entity Recognition via Joint Constrained k-Means and Subspace Selection

Named-entity recognition (NER) is a task that typically requires large annotated datasets, which limits its applicability across domains with varying entity definitions. This paper addresses few-shot NER, aiming to transfer knowledge to new domains with minimal supervision. Unlike previous approaches that rely solely on limited annotated data, we propose a weakly supervised algorithm that combines small labeled datasets with large amounts of unlabeled data. Our method extends the k-means algorithm with label supervision, cluster size constraints and domain-specific discriminative subspace selection. This unified framework achieves state-of-the-art results in few-shot NER on several English datasets.

==> tables/transfer_1_5shot_2_subiterations.tex <==
\begin{table*}[!ht]
    \footnotesize
    \centering
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{Model} & \multicolumn{3}{c}{\textbf{1-shot}} & \multicolumn{3}{c}{\textbf{5-shot}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7}
        & \textbf{CoNLL} & \textbf{WNUT17} & \textbf{Avg.}
        & \textbf{CoNLL} & \textbf{WNUT17} & \textbf{Avg.} \\
        Proto $\dagger$                                & $49.9 {\scriptstyle \pm 8.6} $             & $17.4 {\scriptstyle \pm 4.9}$             & $33.7$             & $61.3 {\scriptstyle \pm 9.1}$             & $22.8 {\scriptstyle \pm 4.5}$             & $42.1$ \\
        NNShot $\dagger$                               & $61.2 {\scriptstyle \pm 10.4}$             & $22.7 {\scriptstyle \pm 7.4}$             & $41.9$             & $74.1 {\scriptstyle \pm 2.3}$             & $27.3 {\scriptstyle \pm 5.4}$             & $50.7$ \\
        StructShot $\dagger$                           & $62.4 {\scriptstyle \pm 10.5}$             & $24.2 {\scriptstyle \pm 8.0}$             & $43.3$             & $74.8 {\scriptstyle \pm 2.4}$             & $30.4 {\scriptstyle \pm 6.5}$             & $52.6$ \\
        CONTaiNER $\dagger$                            & $57.8 {\scriptstyle \pm 10.7}$             & $24.2 {\scriptstyle \pm 2.9}$             & $41.0$             & $72.8 {\scriptstyle \pm 2.0}$             & $27.7 {\scriptstyle \pm 2.2}$             & $50.3$ \\
        ~ + Viterbi $\dagger$                          & $61.2 {\scriptstyle \pm 10.7}$             & $27.5 {\scriptstyle \pm 1.9}$             & $44.4$             & $75.8 {\scriptstyle \pm 2.7}$             & $32.5 {\scriptstyle \pm 3.8}$             & $54.2$ \\
        \midrule
        \multicolumn{7}{l}{\textbf{Discriminative (constrained) K-Means} using unlabeled dev+train} \\
        \midrule
        \multicolumn{7}{l}{\textbf{Hard clustering (\# \texttt{O}-clusters = 10, \# \texttt{I}-clusters = 1)}}
        \\
        \midrule
        \textit{2 sub-iterations} $r_\texttt{O} = NA$  & $65.1 {\scriptstyle \pm 14.0}$             & $22.0 {\scriptstyle \pm  8.3}$             & $43.6$             & $75.3 {\scriptstyle \pm 2.2}$             & $25.1 {\scriptstyle \pm 5.5}$             & $50.2$ \\ 
        $\hookrightarrow \; r_\texttt{O} = 0.80, 0.90$ & $61.6 {\scriptstyle \pm 13.2}$             & $25.0 {\scriptstyle \pm  6.6}$             & $43.3$             & $71.7 {\scriptstyle \pm 3.1}$             & $30.4 {\scriptstyle \pm 3.7}$             & $51.1$ \\ 
        $\hookrightarrow \; r_\texttt{O} = 0.85, 0.95$ & $\underline{65.7 {\scriptstyle \pm 15.9}}$ & $28.5 {\scriptstyle \pm 11.1}$             & $\underline{47.1}$ & $\mathbf{76.6 {\scriptstyle \pm 2.1}}$    & $\mathbf{39.8 {\scriptstyle \pm 3.4}}$    & $\mathbf{58.2}$ \\ 
        \midrule
        \multicolumn{7}{l}{\textbf{Soft clustering (\# \texttt{O}-clusters = 10, \# \texttt{I}-clusters = 1)}}
        \\
        \midrule
        \textit{2 sub-iterations} $r_\texttt{O} = NA$  & $65.1 {\scriptstyle \pm 14.0}$             & $22.9 {\scriptstyle \pm  9.2}$             & $44.0$             & $75.3 {\scriptstyle \pm 2.2}$             & $25.1 {\scriptstyle \pm 5.4}$             & $50.2$ \\ 
        $\hookrightarrow \; r_\texttt{O} = 0.80, 0.95$ & $64.0 {\scriptstyle \pm 15.8}$             & $28.3 {\scriptstyle \pm  9.0}$             & $46.2$             & $74.4 {\scriptstyle \pm 3.5}$             & $36.1 {\scriptstyle \pm 3.5}$             & $55.3$ \\ 
        $\hookrightarrow \; r_\texttt{O} = 0.85, 0.95$ & $63.9 {\scriptstyle \pm 15.7}$             & $\underline{28.7 {\scriptstyle \pm  9.4}}$ & $46.3$             & $74.3 {\scriptstyle \pm 3.5}$             & $36.2 {\scriptstyle \pm 3.6}$             & $55.3$ \\ 
        \midrule
        \multicolumn{7}{l}{\textbf{Using unlabeled dev set only}} \\
        \midrule
        \multicolumn{7}{l}{\textbf{Hard clustering (\# \texttt{O}-clusters = 10, \# \texttt{I}-clusters = 1)}}
        \\
        \midrule
        \textit{2 sub-iterations} $r_\texttt{O} = NA$  & $64.2 {\scriptstyle \pm 15.1}$             & $20.4 {\scriptstyle \pm  8.0}$             & $42.3$             & $74.2 {\scriptstyle \pm  2.4}$              & $25.4 {\scriptstyle \pm  4.6}$             & $49.8$ \\ 
        $\hookrightarrow \; r_\texttt{O} = 0.80, 0.90$ & $61.1 {\scriptstyle \pm 14.1}$             & $21.2 {\scriptstyle \pm  6.1}$             & $41.2$             & $70.4 {\scriptstyle \pm  2.9}$              & $24.9 {\scriptstyle \pm  3.1}$             & $47.7$ \\ 
        $\hookrightarrow \; r_\texttt{O} = 0.85, 0.95$ & $65.5 {\scriptstyle \pm 14.9}$             & $\mathbf{28.4 {\scriptstyle \pm  9.8}}$    & $\mathbf{47.0}$    & $\underline{75.4 {\scriptstyle \pm  2.6}}$  & $\underline{38.2 {\scriptstyle \pm  3.3}}$ & $\underline{56.8}$ \\ 
        \midrule
        \multicolumn{7}{l}{\textbf{Soft clustering (\# \texttt{O}-clusters = 10, \# \texttt{I}-clusters = 1)}}
        \\
        \midrule
        \textit{2 sub-iterations} $r_\texttt{O} = NA$  & $64.4 {\scriptstyle \pm 15.1}$             & $20.3 {\scriptstyle \pm  8.2}$             & $42.4$             & $74.2 {\scriptstyle \pm  2.4}$              & $25.4 {\scriptstyle \pm  4.4}$             & $49.8$ \\ 
        $\hookrightarrow \; r_\texttt{O} = 0.80, 0.90$ & $64.4 {\scriptstyle \pm 15.0}$             & $27.5 {\scriptstyle \pm 10.5}$             & $46.0$             & $73.2 {\scriptstyle \pm  2.7}$              & $35.9 {\scriptstyle \pm  3.9}$             & $54.6$ \\ 
        $\hookrightarrow \; r_\texttt{O} = 0.85, 0.95$ & $64.4 {\scriptstyle \pm 14.9}$             & $27.7 {\scriptstyle \pm 10.5}$             & $\underline{46.1}$ & $73.1 {\scriptstyle \pm  2.8}$              & $36.1 {\scriptstyle \pm  3.7}$             & $54.6$ \\ 
        \midrule
        \multicolumn{7}{l}{\textbf{Discriminative (constrained) K-Means using the support sets only}} \\
        \midrule
        \multicolumn{7}{l}{\textbf{Discriminative (constrained) K-Means (\# \texttt{O}-clusters = 10, \# \texttt{I}-clusters = 1)}} \\
        \midrule
        \# \texttt{I}-clusters = 1 & $63.8 {\scriptstyle \pm 8.7}$ & $21.0 {\scriptstyle \pm 10.4}$ & $42.4$ & $73.5 {\scriptstyle \pm 3.7}$ & $32.3 {\scriptstyle \pm 4.3}$ & $52.9$ \\
        \bottomrule
    \end{tabular}
    \caption{F1 scores in domain adaptation with OntoNotes as the source domain. Results marked with $\dagger$ for existing models are taken from \citet{das-2022-container-contrastive} and evaluation of our proposed method is done on the same 10 supports.
    Ratio constraints are noted in the order of datasets, e.g.\ $r_\texttt{O} = 0.80, 0.90$ means that the first dataset, CoNLL, is tested with a ratio of $0.80$ and the second dataset, WNUT17, is tested with a ratio of $0.90$. }
    \label{tab:main-results}
\end{table*}

